Towards Leveraging News Media to Support Impact Assessment of AI Technologies

Expert-driven frameworks for impact assessments (IAs) may inadvertently overlook the effects of AI technologies on the public's social behavior, policy, and the cultural and geographical contexts shaping the perception of AI and the impacts around its use. This research explores the potentials of fine-tuning LLMs on negative impacts of AI reported in a diverse sample of articles from 266 news domains spanning 30 countries around the world to incorporate more diversity into IAs. Our findings highlight (1) the potential of fine-tuned open-source LLMs in supporting IA of AI technologies by generating high-quality negative impacts across four qualitative dimensions: coherence, structure, relevance, and plausibility, and (2) the efficacy of small open-source LLM (Mistral-7B) fine-tuned on impacts from news media in capturing a wider range of categories of impacts that GPT-4 had gaps in covering.

==> conclusion.tex <==
Our work demonstrates the potential for generating high-quality and diverse impacts of
AI in society by fine-tuning completion models (GPT-3 and Mistral-7B) on a diverse sample of articles from news media and comparing those outputs to the impacts generated by instruction-based (GPT-4 and Mistral-7B-Instruct) models. We examine the generated impacts for coherence, structure, relevance, and plausibility and find that the generated impacts using Mistral-7B, a small open-source model finetuned on impacts from the news media, tend to be qualitatively on par with impacts generated using a more capable and larger scale model such as GPT-4. Moreover, we find that impacts produced by instruction-based models had gaps in the production of certain categories of impacts in comparison to fine-tuned models. This research highlights a potential bias in the range of impacts generated by state-of-the-art LLMs and
the potential of aligning smaller LLMs on news media as a scalable alternative to generate high quality and more diverse impacts in support of anticipatory governance approaches.

==> data.tex <==
Our dataset consists of 91,930 articles in English retrieved and then scraped from Google News using a curated set of 40 AI-relevant keywords (as listed in \ref{a.1}) that were published by 266 domains between January 1, 2020 and June 1st 2023 spanning 30 countries around the world (see \ref{a.2} for the distribution of articles for the top 10 countries).

==> refs.tex <==
@misc{solaiman_evaluating_2023,
  title = {Evaluating the {Social} {Impact} of {Generative} {AI} {Systems} in {Systems} and {Society}},
  url = {http://arxiv.org/abs/2306.05949},
  abstract = {Generative AI systems across modalities, ranging from text, image, audio, and video, have broad social impacts, but there exists no official standard for means of evaluating those impacts and which impacts should be evaluated. We move toward a standard approach in evaluating a generative AI system for any modality, in two overarching categories: what is able to be evaluated in a base system that has no predetermined application and what is able to be evaluated in society. We describe specific social impact categories and how to approach and conduct evaluations in the base technical system, then in people and society. Our framework for a base system defines seven categories of social impact: bias, stereotypes, and representational harms; cultural values and sensitive content; disparate performance; privacy and data protection; financial costs; environmental costs; and data and content moderation labor costs. Suggested methods for evaluation apply to all modalities and analyses of the limitations of existing evaluations serve as a starting point for necessary investment in future evaluations. We offer five overarching categories for what is able to be evaluated in society, each with their own subcategories: trustworthiness and autonomy; inequality, marginalization, and violence; concentration of authority; labor and creativity; and ecosystem and environment. Each subcategory includes recommendations for mitigating harm. We are concurrently crafting an evaluation repository for the AI research community to contribute existing evaluations along the given categories. This version will be updated following a CRAFT session at ACM FAccT 2023.},
  urldate = {2023-07-18},
  publisher = {arXiv},
  author = {Solaiman, Irene and Talat, Zeerak and Agnew, William and Ahmad, Lama and Baker, Dylan and Blodgett, Su Lin and Daumé III, Hal and Dodge, Jesse and Evans, Ellie and Hooker, Sara and Jernite, Yacine and Luccioni, Alexandra Sasha and Lusoli, Alberto and Mitchell, Margaret and Newman, Jessica and Png, Marie-Therese and Strait, Andrew and Vassilev, Apostol},
  month = jun,
  year = {2023},
  note = {arXiv:2306.05949 [cs]},
  keywords = {Computer Science - Computers and Society, Computer Science - Artificial Intelligence},
  file = {arXiv.org Snapshot:/Users/Mowafak/Zotero/storage/95J82WWN/2306.html:text/html;Full Text PDF:/Users/Mowafak/Zotero/storage/L79YHJIL/Solaiman et al. - 2023 - Evaluating the Social Impact of Generative AI Syst.pdf:application/pdf},
}

@inproceedings{metcalf_algorithmic_2021,
  address = {Virtual Event Canada},
  title = {Algorithmic {Impact} {Assessments} and {Accountability}: {The} {Co}-construction of {Impacts}},
  isbn = {978-1-4503-8309-7},
  shorttitle = {Algorithmic {Impact} {Assessments} and {Accountability}},
  url = {https://dl.acm.org/doi/10.1145/3442188.3445935},
  doi = {10.1145/3442188.3445935},
  language = {en},
  urldate = {2023-10-16},
  booktitle = {Proceedings of the 2021 {ACM} {Conference} on {Fairness}, {Accountability}, and {Transparency}},
  publisher = {ACM},
  author = {Metcalf, Jacob and Moss, Emanuel and Watkins, Elizabeth Anne and Singh, Ranjit and Elish, Madeleine Clare},
  month = mar,
  year = {2021},
  pages = {735--746},
  file = {Full Text PDF:/Users/Mowafak/Zotero/storage/SNYM5DIA/Metcalf et al. - 2021 - Algorithmic Impact Assessments and Accountability.pdf:application/pdf},
}

@article{DBLP:journals/corr/abs-2011-13170,
  author       = {Priyanka Nanayakkara and
                  Nicholas Diakopoulos and
                  Jessica Hullman},
  title        = {Anticipatory Ethics and the Role of Uncertainty},
  journal      = {CoRR},
  volume       = {abs/2011.13170},
  year         = {2020},
  url          = {https://arxiv.org/abs/2011.13170},
  eprinttype    = {arXiv},
  eprint       = {2011.13170},
  timestamp    = {Tue, 01 Dec 2020 14:59:59 +0100},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2011-13170.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@misc{schuett_towards_2023,
  title = {Towards best practices in {AGI} safety and governance: {A} survey of expert opinion},
  shorttitle = {Towards best practices in {AGI} safety and governance},
  url = {http://arxiv.org/abs/2305.07153},
  abstract = {A number of leading AI companies, including OpenAI, Google DeepMind, and Anthropic, have the stated goal of building artificial general intelligence (AGI) - AI systems that achieve or exceed human performance across a wide range of cognitive tasks. In pursuing this goal, they may develop and deploy AI systems that pose particularly significant risks. While they have already taken some measures to mitigate these risks, best practices have not yet emerged. To support the identification of best practices, we sent a survey to 92 leading experts from AGI labs, academia, and civil society and received 51 responses. Participants were asked how much they agreed with 50 statements about what AGI labs should do. Our main finding is that participants, on average, agreed with all of them. Many statements received extremely high levels of agreement. For example, 98\% of respondents somewhat or strongly agreed that AGI labs should conduct pre-deployment risk assessments, dangerous capabilities evaluations, third-party model audits, safety restrictions on model usage, and red teaming. Ultimately, our list of statements may serve as a helpful foundation for efforts to develop best practices, standards, and regulations for AGI labs.},
  urldate = {2023-06-13},
  publisher = {arXiv},
  author = {Schuett, Jonas and Dreksler, Noemi and Anderljung, Markus and McCaffary, David and Heim, Lennart and Bluemke, Emma and Garfinkel, Ben},
  month = may,
  year = {2023},
  note = {arXiv:2305.07153 [cs]},
  keywords = {Computer Science - Computers and Society},
  file = {arXiv.org Snapshot:/Users/Mowafak/Zotero/storage/D4AUWY8I/2305.html:text/html;Full Text PDF:/Users/Mowafak/Zotero/storage/HE59RVJU/Schuett et al. - 2023 - Towards best practices in AGI safety and governanc.pdf:application/pdf},
}
@article{DBLP:journals/corr/abs-2108-07258,
  author       = {Rishi Bommasani and
                  Drew A. Hudson and
                  Ehsan Adeli and
                  Russ B. Altman and
                  Simran Arora and
                  Sydney von Arx and
                  Michael S. Bernstein and
                  Jeannette Bohg and
                  Antoine Bosselut and
                  Emma Brunskill and
                  Erik Brynjolfsson and
                  Shyamal Buch and
                  Dallas Card and
                  Rodrigo Castellon and
                  Niladri S. Chatterji and
                  Annie S. Chen and
                  Kathleen Creel and
                  Jared Quincy Davis and
                  Dorottya Demszky and
                  Chris Donahue and
                  Moussa Doumbouya and
                  Esin Durmus and
                  Stefano Ermon and
                  John Etchemendy and
                  Kawin Ethayarajh and
                  Li Fei{-}Fei and
                  Chelsea Finn and
                  Trevor Gale and
                  Lauren Gillespie and
                  Karan Goel and
                  Noah D. Goodman and
                  Shelby Grossman and
                  Neel Guha and
                  Tatsunori Hashimoto and
                  Peter Henderson and
                  John Hewitt and
                  Daniel E. Ho and
                  Jenny Hong and
                  Kyle Hsu and
                  Jing Huang and
                  Thomas Icard and
                  Saahil Jain and
                  Dan Jurafsky and
                  Pratyusha Kalluri and
                  Siddharth Karamcheti and
                  Geoff Keeling and
                  Fereshte Khani and
                  Omar Khattab and
                  Pang Wei Koh and
                  Mark S. Krass and
                  Ranjay Krishna and
                  Rohith Kuditipudi and
                  et al.},
  title        = {On the Opportunities and Risks of Foundation Models},
  journal      = {CoRR},
  volume       = {abs/2108.07258},
  year         = {2021},
  url          = {https://arxiv.org/abs/2108.07258},
  eprinttype    = {arXiv},
  eprint       = {2108.07258},
  timestamp    = {Fri, 17 Feb 2023 09:02:02 +0100},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2108-07258.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{weidinger_taxonomy_2022,
  address = {Seoul Republic of Korea},
  title = {Taxonomy of {Risks} posed by {Language} {Models}},
  isbn = {978-1-4503-9352-2},
  url = {https://dl.acm.org/doi/10.1145/3531146.3533088},
  doi = {10.1145/3531146.3533088},
  language = {en},
  urldate = {2023-10-16},
  booktitle = {2022 {ACM} {Conference} on {Fairness}, {Accountability}, and {Transparency}},
  publisher = {ACM},
  author = {Weidinger, Laura and Uesato, Jonathan and Rauh, Maribeth and Griffin, Conor and Huang, Po-Sen and Mellor, John and Glaese, Amelia and Cheng, Myra and Balle, Borja and Kasirzadeh, Atoosa and Biles, Courtney and Brown, Sasha and Kenton, Zac and Hawkins, Will and Stepleton, Tom and Birhane, Abeba and Hendricks, Lisa Anne and Rimell, Laura and Isaac, William and Haas, Julia and Legassick, Sean and Irving, Geoffrey and Gabriel, Iason},
  month = jun,
  year = {2022},
  pages = {214--229},
  file = {Full Text PDF:/Users/Mowafak/Zotero/storage/XBZ2SKI8/Weidinger et al. - 2022 - Taxonomy of Risks posed by Language Models.pdf:application/pdf},
}

@inproceedings{nanayakkara_unpacking_2021,
  address = {Virtual Event USA},
  title = {Unpacking the {Expressed} {Consequences} of {AI} {Research} in {Broader} {Impact} {Statements}},
  isbn = {978-1-4503-8473-5},
  url = {https://dl.acm.org/doi/10.1145/3461702.3462608},
  doi = {10.1145/3461702.3462608},
  language = {en},
  urldate = {2023-10-16},
  booktitle = {Proceedings of the 2021 {AAAI}/{ACM} {Conference} on {AI}, {Ethics}, and {Society}},
  publisher = {ACM},
  author = {Nanayakkara, Priyanka and Hullman, Jessica and Diakopoulos, Nicholas},
  month = jul,
  year = {2021},
  pages = {795--806},
  file = {Full Text PDF:/Users/Mowafak/Zotero/storage/W4RRXH5Z/Nanayakkara et al. - 2021 - Unpacking the Expressed Consequences of AI Researc.pdf:application/pdf},
}

@article{bonaccorsi2020expert,
  title={Expert biases in technology foresight. Why they are a problem and how to mitigate them},
  author={Bonaccorsi, Andrea and Apreda, Riccardo and Fantoni, Gualtiero},
  journal={Technological Forecasting and Social Change},
  volume={151},
  pages={119855},
  year={2020},
  publisher={Elsevier}
}

@article{crawford2016artificial,
  title={Artificial intelligence’s white guy problem},
  author={Crawford, Kate},
  journal={The New York Times},
  volume={25},
  number={06},
  pages={5},
  year={2016}
}

@inproceedings{10.1145/3306618.3314285,
author = {Chuan, Ching-Hua and Tsai, Wan-Hsiu Sunny and Cho, Su Yeon},
title = {Framing Artificial Intelligence in American Newspapers},
year = {2019},
isbn = {9781450363242},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3306618.3314285},
doi = {10.1145/3306618.3314285},
abstract = {Publics' perceptions of new scientific advances such as AI are often informed and influenced by news coverage. To understand how artificial intelligence (AI) was framed in U.S. newspapers, a content analysis based on framing theory in journalism and science communication was conducted. This study identified the dominant topics and frames, as well as the risks and benefits of AI covered in five major American newspapers from 2009 to 2018. Results indicated that business and technology were the primary topics in news coverage of AI. The benefits of AI were discussed more frequently than its risks, but risks of AI were generally discussed with greater specificity. Additionally, episodic issue framing and societal impact framing were more frequently used.},
booktitle = {Proceedings of the 2019 AAAI/ACM Conference on AI, Ethics, and Society},
pages = {339–344},
numpages = {6},
keywords = {content analysis, artificial intelligence, public perception, news framing},
location = {Honolulu, HI, USA},
series = {AIES '19}
}

@article{nguyen2022news,
  title={The news framing of artificial intelligence: a critical exploration of how media discourses make sense of automation},
  author={Nguyen, Dennis and Hekman, Erik},
  journal={Ai \& Society},
  pages={1--15},
  year={2022},
  publisher={Springer}
}

@article{diakopoulos2024prospective,
    author = {Nicholas Diakopoulos},
    title = {Prospective Algorithmic Accountability and the Role of the News Media},
    booktitle = {Computer Ethics Across Disciplines: Applying Deborah Johnson’s Philosophy to Algorithmic Accountability and AI},
    publisher = {Springer},
    year = {2024},
    editor = {Merel Noorman and Mario Verdicchio},
    chapter = {}
}

@article{metag2014technophobia,
  title={Technophobia towards emerging technologies? A comparative analysis of the media coverage of nanotechnology in Austria, Switzerland and Germany},
  author={Metag, Julia and Marcinkowski, Frank},
  journal={Journalism},
  volume={15},
  number={4},
  pages={463--481},
  year={2014},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{ouchchy2020ai,
  title={AI in the headlines: the portrayal of the ethical issues of artificial intelligence in the media},
  author={Ouchchy, Leila and Coin, Allen and Dubljevi{\'c}, Veljko},
  journal={AI \& SOCIETY},
  volume={35},
  pages={927--936},
  year={2020},
  publisher={Springer}
}

@misc{brennen2018industry,
  title={An industry-led debate: How UK media cover artificial intelligence. RISJ Fact-Sheet},
  author={Brennen, JS and Howard, Philip N and Nielsen, Rasmus Kleis},
  year={2018},
  publisher={Oxford, UK: University of Oxford}
}

@article{sun2020newspaper,
  title={Newspaper coverage of artificial intelligence: A perspective of emerging technologies},
  author={Sun, Shaojing and Zhai, Yujia and Shen, Bin and Chen, Yibei},
  journal={Telematics and Informatics},
  volume={53},
  pages={101433},
  year={2020},
  publisher={Elsevier}
}

@article{10.1162/tacl_a_00632,
    author = {Zhang, Tianyi and Ladhak, Faisal and Durmus, Esin and Liang, Percy and McKeown, Kathleen and Hashimoto, Tatsunori B.},
    title = "{Benchmarking Large Language Models for News Summarization}",
    journal = {Transactions of the Association for Computational Linguistics},
    volume = {12},
    pages = {39-57},
    year = {2024},
    month = {01},
    abstract = "{Large language models (LLMs) have shown promise for automatic summarization but the reasons behind their successes are poorly understood. By conducting a human evaluation on ten LLMs across different pretraining methods, prompts, and model scales, we make two important observations. First, we find instruction tuning, not model size, is the key to the LLM’s zero-shot summarization capability. Second, existing studies have been limited by low-quality references, leading to underestimates of human performance and lower few-shot and finetuning performance. To better evaluate LLMs, we perform human evaluation over high-quality summaries we collect from freelance writers. Despite major stylistic differences such as the amount of paraphrasing, we find that LLM summaries are judged to be on par with human written summaries.}",
    issn = {2307-387X},
    doi = {10.1162/tacl_a_00632},
    url = {https://doi.org/10.1162/tacl\_a\_00632},
    eprint = {https://direct.mit.edu/tacl/article-pdf/doi/10.1162/tacl\_a\_00632/2325685/tacl\_a\_00632.pdf},
}

@article{grootendorst2022bertopic,
  title={BERTopic: Neural topic modeling with a class-based TF-IDF procedure},
  author={Grootendorst, Maarten},
  journal={arXiv preprint arXiv:2203.05794},
  year={2022}
}

@misc{jiang2023mistral,
      title={Mistral 7B}, 
      author={Albert Q. Jiang and Alexandre Sablayrolles and Arthur Mensch and Chris Bamford and Devendra Singh Chaplot and Diego de las Casas and Florian Bressand and Gianna Lengyel and Guillaume Lample and Lucile Saulnier and Lélio Renard Lavaud and Marie-Anne Lachaux and Pierre Stock and Teven Le Scao and Thibaut Lavril and Thomas Wang and Timothée Lacroix and William El Sayed},
      year={2023},
      eprint={2310.06825},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{dettmers2023qlora,
      title={QLoRA: Efficient Finetuning of Quantized LLMs}, 
      author={Tim Dettmers and Artidoro Pagnoni and Ari Holtzman and Luke Zettlemoyer},
      year={2023},
      eprint={2305.14314},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{herdel2024exploregen,
  title={ExploreGen: Large Language Models for Envisioning the Uses and Risks of AI Technologies},
  author={Herdel, Viviane and {\v{S}}{\'c}epanovi{\'c}, Sanja and Bogucka, Edyta and Quercia, Daniele},
  journal={arXiv preprint arXiv:2407.12454},
  year={2024}
}
@article{navigli2023biases,
  title={Biases in large language models: origins, inventory, and discussion},
  author={Navigli, Roberto and Conia, Simone and Ross, Bj{\"o}rn},
  journal={ACM Journal of Data and Information Quality},
  volume={15},
  number={2},
  pages={1--21},
  year={2023},
  publisher={ACM New York, NY}
}

@inproceedings{talat2022you,
  title={You reap what you sow: On the challenges of bias evaluation under multilingual settings},
  author={Talat, Zeerak and N{\'e}v{\'e}ol, Aur{\'e}lie and Biderman, Stella and Clinciu, Miruna and Dey, Manan and Longpre, Shayne and Luccioni, Sasha and Masoud, Maraim and Mitchell, Margaret and Radev, Dragomir and others},
  booktitle={Proceedings of BigScience Episode\# 5--Workshop on Challenges \& Perspectives in Creating Large Language Models},
  pages={26--41},
  year={2022}
}

@misc{shelby_sociotechnical_2023,
  title = {Sociotechnical {Harms} of {Algorithmic} {Systems}: {Scoping} a {Taxonomy} for {Harm} {Reduction}},
  shorttitle = {Sociotechnical {Harms} of {Algorithmic} {Systems}},
  url = {http://arxiv.org/abs/2210.05791},
  abstract = {Understanding the landscape of potential harms from algorithmic systems enables practitioners to better anticipate consequences of the systems they build. It also supports the prospect of incorporating controls to help minimize harms that emerge from the interplay of technologies and social and cultural dynamics. A growing body of scholarship has identified a wide range of harms across different algorithmic technologies. However, computing research and practitioners lack a high level and synthesized overview of harms from algorithmic systems. Based on a scoping review of computing research \$(n=172)\$, we present an applied taxonomy of sociotechnical harms to support a more systematic surfacing of potential harms in algorithmic systems. The final taxonomy builds on and refers to existing taxonomies, classifications, and terminologies. Five major themes related to sociotechnical harms - representational, allocative, quality-of-service, interpersonal harms, and social system/societal harms - and sub-themes are presented along with a description of these categories. We conclude with a discussion of challenges and opportunities for future research.},
  urldate = {2023-08-13},
  publisher = {arXiv},
  author = {Shelby, Renee and Rismani, Shalaleh and Henne, Kathryn and Moon, AJung and Rostamzadeh, Negar and Nicholas, Paul and Yilla, N'Mah and Gallegos, Jess and Smart, Andrew and Garcia, Emilio and Virk, Gurleen},
  month = jul,
  year = {2023},
  note = {arXiv:2210.05791 [cs]},
  keywords = {Computer Science - Human-Computer Interaction, Computer Science - General Literature},
  file = {arXiv.org Snapshot:/Users/Mowafak/Zotero/storage/VTCY7HRU/2210.html:text/html;Full Text PDF:/Users/Mowafak/Zotero/storage/TJVQPEKP/Shelby et al. - 2023 - Sociotechnical Harms of Algorithmic Systems Scopi.pdf:application/pdf},
}

@article{kieslich2024ever,
  title={Ever heard of ethical AI? Investigating the salience of ethical AI issues among the German population},
  author={Kieslich, Kimon and L{\"u}nich, Marco and Do{\v{s}}enovi{\'c}, Pero},
  journal={International Journal of Human--Computer Interaction},
  volume={40},
  number={11},
  pages={2986--2999},
  year={2024},
  publisher={Taylor \& Francis}
}

@inproceedings{kieslich2024regulating,
  title={Regulating AI-Based Remote Biometric Identification. Investigating the Public Demand for Bans, Audits, and Public Database Registrations},
  author={Kieslich, Kimon and L{\"u}nich, Marco},
  booktitle={The 2024 ACM Conference on Fairness, Accountability, and Transparency},
  pages={173--185},
  year={2024}
}

@article{uruena2019understanding,
  title={Understanding “plausibility”: A relational approach to the anticipatory heuristics of future scenarios},
  author={Urue{\~n}a, Sergio},
  journal={Futures},
  volume={111},
  pages={15--25},
  year={2019},
  publisher={Elsevier}
}

@article{diakopoulos2021anticipating,
  title={Anticipating and addressing the ethical implications of deepfakes in the context of elections},
  author={Diakopoulos, Nicholas and Johnson, Deborah},
  journal={New media \& society},
  volume={23},
  number={7},
  pages={2072--2098},
  year={2021},
  publisher={Sage Publications Sage UK: London, England}
}

@article{buccinca2023aha,
  title={Aha!: Facilitating ai impact assessment by generating examples of harms},
  author={Bu{\c{c}}inca, Zana and Pham, Chau Minh and Jakesch, Maurice and Ribeiro, Marco Tulio and Olteanu, Alexandra and Amershi, Saleema},
  journal={arXiv preprint arXiv:2306.03280},
  year={2023}
}

@inproceedings{pang2024blip,
  title={BLIP: Facilitating the Exploration of Undesirable Consequences of Digital Technologies},
  author={Pang, Rock Yuren and Santy, Sebastin and Just, Ren{\'e} and Reinecke, Katharina},
  booktitle={Proceedings of the CHI Conference on Human Factors in Computing Systems},
  pages={1--18},
  year={2024}
}

@article{dsa_observatory_2024,
  title={What do we talk about when we talk about risk? Risk politics in the EU’s Digital Services Act},
  author={{DSA Observatory}},
  year={2024},
  url={https://dsa-observatory.eu/2024/07/31/what-do-we-talk-about-when-we-talk-about-risk-risk-politics-in-the-eus-digital-services-act/},
  note={Accessed: 2024-09-19}
}

